Guard Your Daggers and Traces: On The Equational Properties of Guarded (Co-)recursion

Motivated by the recent interest in models of guarded (co-)recursion we study its equational properties. We formulate axioms for guarded fixpoint operators generalizing the axioms of iteration theories of Bloom and Esik. Models of these axioms include both standard (e.g., cpo-based) models of iteration theories and models of guarded recursion such as complete metric spaces or the topos of trees studied by Birkedal et al. We show that the standard result on the satisfaction of all Conway axioms by a unique dagger operation generalizes to the guarded setting. We also introduce the notion of guarded trace operator on a category, and we prove that guarded trace and guarded fixpoint operators are in one-to-one correspondence. Our results are intended as first steps leading to the description of classifying theories for guarded recursion and hence completeness results involving our axioms of guarded fixpoint operators in future work.

==> eptcsdata.tex <==
\providecommand{\firstpage}{72}
\providecommand{\publicationstatus}{D. Baelde and A. Carayol (Eds.): Fixed Points\\
in Computer Science 2013 (FICS 2013)\\
EPTCS 126, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.126.6}{10.4204/EPTCS.126.6}}
\pdfoutput=1

